SP2: A Second Order Stochastic Polyak Method

Recently the "SP" (Stochastic Polyak step size) method has emerged as a competitive adaptive method for setting the step sizes of SGD. SP can be interpreted as a method specialized to interpolated models, since it solves the interpolation equations. SP solves these equation by using local linearizations of the model. We take a step further and develop a method for solving the interpolation equations that uses the local second-order approximation of the model. Our resulting method SP2 uses Hessian-vector products to speed-up the convergence of SP. Furthermore, and rather uniquely among second-order methods, the design of SP2 in no way relies on positive definite Hessian matrices or convexity of the objective function. We show SP2 is very competitive on matrix completion, non-convex test problems and logistic regression. We also provide a convergence theory on sums-of-quadratics.

==> header.tex <==
 % style
\usepackage{fullpage}
\usepackage{layout}
\usepackage{multirow}
% \usepackage{cases}

\usepackage{bm,bbm,amssymb,amsthm,graphicx}

% ams
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb} % NOT COMPATIBLE WITH svjour3

% references
\usepackage{hyperref}

% clever references
\usepackage{cleveref}


% nice fractions
\usepackage{nicefrac}
\usepackage{mathtools}

% system with left brace and one label per line
\usepackage{empheq}

\newcommand{\colvec}[1]{\begin{bmatrix}#1\end{bmatrix}}

%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Normal THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%
%\newtheorem{assumption}{Assumption}
%\newtheorem{lemma}{Lemma}
%\newtheorem{algorithms}{Algorithm}
%\newtheorem{theorem}{Theorem}
%\newtheorem{proposition}{Proposition}
%\newtheorem{example}{Example}
%\newtheorem{remark}{Remark}
%\newtheorem{claim}[theorem]{Claim}
%\newtheorem{corollary}{Corollary}
%\newtheorem{exercise}[theorem]{Exercise}
%
%\theoremstyle{definition}
%\newtheorem{definition}[theorem]{Definition}


%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% shaded THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{mdframed}
\usepackage{thmtools}

\definecolor{shadecolor}{gray}{0.90}
\declaretheoremstyle[
headfont=\normalfont\bfseries,
notefont=\mdseries, notebraces={(}{)},
bodyfont=\normalfont,
postheadspace=0.5em,
spaceabove=1pt,
mdframed={
  skipabove=8pt,
  skipbelow=8pt,
  hidealllines=true,
  backgroundcolor={shadecolor},
  innerleftmargin=4pt,
  innerrightmargin=4pt}
]{shaded}


\declaretheorem[style=shaded,within=section]{definition}
\declaretheorem[style=shaded,sibling=definition]{theorem}
\declaretheorem[style=shaded,sibling=definition]{proposition}
\declaretheorem[style=shaded,sibling=definition]{assumption}
\declaretheorem[style=shaded,sibling=definition]{corollary}
\declaretheorem[style=shaded,sibling=definition]{conjecture}
\declaretheorem[style=shaded,sibling=definition]{lemma}
\declaretheorem[style=shaded,sibling=definition]{remark}
\declaretheorem[style=shaded,sibling=definition]{example}

% Names used by cleveref's \Cref command
\crefname{assumption}{assumption}{assumptions}


% algorithms
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}



% captions
% \usepackage{caption}
% \usepackage{subcaption}


% graphics
 \usepackage{xcolor}
\usepackage{color}
\usepackage{graphicx}
\graphicspath{{./figures/}}  % Path to figures folder


% various
%\usepackage[cp1250]{inputenc}
%\usepackage[T1]{fontenc}


\newcommand\tagthis{\addtocounter{equation}{1}\tag{\theequation}}

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% BIBLIOGRAPHY
%%%%%%%%%%%%%%%%%%%%%%%%%

%\usepackage[maxbibnames=99, maxcitenames=10,doi=false,isbn=false,url=false,backend=bibtex]{biblatex}
%%\bibliography{SDA.bib}
%\newcommand{\Ref}[1]{../ref/#1}
%%\input{\Ref{biblatex_journal_def}}

%%% Basic sets
\newcommand{\R}{\mathbb{R}} % Reals
\newcommand{\N}{\mathbb{N}} % Naturals

% caligraphic
\newcommand{\cA}{{\cal A}}
\newcommand{\cB}{{\cal B}}
\newcommand{\cC}{{\cal C}}
\newcommand{\cD}{{\cal D}}
\newcommand{\cE}{{\cal E}}
\newcommand{\cF}{{\cal F}}
\newcommand{\cG}{{\cal G}}
\newcommand{\cH}{{\cal H}}
\newcommand{\cJ}{{\cal J}}
\newcommand{\cK}{{\cal K}}
\newcommand{\cL}{{\cal L}}
\newcommand{\cM}{{\cal M}}
\newcommand{\cN}{{\cal N}}
\newcommand{\cO}{{\cal O}}
\newcommand{\cP}{{\cal P}}
\newcommand{\cQ}{{\cal Q}}
\newcommand{\cR}{{\cal R}}
\newcommand{\cS}{{\cal S}}
\newcommand{\cT}{{\cal T}}
\newcommand{\cU}{{\cal U}}
\newcommand{\cV}{{\cal V}}
\newcommand{\cX}{{\cal X}}
\newcommand{\cY}{{\cal Y}}
\newcommand{\cW}{{\cal W}}
\newcommand{\cZ}{{\cal Z}}


% bold
\newcommand{\bA}{{\bf A}}
\newcommand{\bB}{{\bf B}}
\newcommand{\bC}{{\bf C}}
\newcommand{\bE}{{\bf E}}
\newcommand{\bI}{{\bf I}}
\newcommand{\bS}{{\bf S}}
\newcommand{\bZ}{{\bf Z}}

% vectors
\def \va {\bm{a}}
\def \vb {\bm{b}}
\def \vc {\bm{c}}
\def \vg {\bm{g}}
\def \vvh {\bm{h}}
\def \vu {\bm{u}}
\def \vv {\bm{v}}
\def \vw {\bm{w}}
\def \vx {\bm{x}}
\def \vz {\bm{z}}


\def \stt {\operatorname*{s.t. }}

% matrices
\newcommand{\mA}{{\bf A}}
\newcommand{\mB}{{\bf B}}
\newcommand{\mC}{{\bf C}}
\newcommand{\mD}{{\bf D}}

\newcommand{\mE}{{\bf E}}
\newcommand{\mF}{{\bf F}}
\newcommand{\mG}{{\bf G}}
\newcommand{\mH}{{\bf H}}
\newcommand{\mI}{{\bf I}}
\newcommand{\mJ}{{\bf J}}
\newcommand{\mK}{{\bf K}}
\newcommand{\mL}{{\bf L}}
\newcommand{\mM}{{\bf M}}
\newcommand{\mN}{{\bf N}}
\newcommand{\mO}{{\bf O}}
\newcommand{\mP}{{\bf P}}
\newcommand{\mQ}{{\bf Q}}
\newcommand{\mR}{{\bf R}}
\newcommand{\mS}{{\bf S}}
\newcommand{\mT}{{\bf T}}
\newcommand{\mU}{{\bf U}}
\newcommand{\mV}{{\bf V}}
\newcommand{\mW}{{\bf W}}
\newcommand{\mX}{{\bf X}}
\newcommand{\mY}{{\bf Y}}
\newcommand{\mZ}{{\bf Z}}
\newcommand{\mLambda}{{\bf \Lambda}}

\newcommand{\zeros}{{\bf 0}}
\newcommand{\ones}{{\bf 1}}

\newcommand{\LF}{{\mathcal{L}}}


\newcommand{\ut}{{\widetilde{u}}}
\newcommand{\uh}{{\widehat{u}}}
\newcommand{\Uh}{{\widehat{\mU}}}
\newcommand{\vh}{{\hat{v}}}
\newcommand{\wh}{{\hat{w}}}

%Will
\newcommand{\inner}[2]{\left\langle #1, #2 \right\rangle}



% Commenting
% \usepackage[dvipsnames]{xcolor}  % Coloured text etc.
\usepackage[colorinlistoftodos,bordercolor=orange,backgroundcolor=orange!20,linecolor=orange,textsize=scriptsize]{todonotes}
\newcommand{\TODO}[1]{\todo[inline,linecolor=green,backgroundcolor=green!25,bordercolor=green,caption={}]{#1}}
\newcommand{\rob}[1]{\todo[inline]{\textbf{Robert: }#1}}
\newcommand{\will}[1]{\todo[inline]{\textbf{Will: }#1}}
\newcommand{\MT}[1]{\todo[inline,linecolor=red,backgroundcolor=red!25,bordercolor=red]{\textbf{MT: }#1}}
\newcommand{\SL}[1]{\todo[inline,linecolor=blue,backgroundcolor=blue!25,bordercolor=blue]{\textbf{SL: }#1}}


% basic
% \newcommand{\eqdef}{\overset{\text{def}}{=}}
\newcommand{\eqdef}{\coloneqq}

%\newcommand{\eqdef}{\stackrel{\text{def}}{=}}
\newcommand{\st}{\;:\;} % such that
\newcommand{\ve}[2]{\langle #1 ,  #2 \rangle} % inner
\newcommand{\dotprod}[1]{\left< #1\right>} % product
\newcommand{\norm}[1]{ \left\| #1 \right\|}      % norm


% statistical
%\DeclareMathOperator{\Exp}{\mathbf{E}} % expectation
\DeclareMathOperator{\Cov}{Cov}         % covariance
\DeclareMathOperator{\Var}{Var}         % variance
\DeclareMathOperator{\Corr}{Corr}       % correlation
\DeclareMathOperator{\nnz}{nnz}       % number of non zeros.
%\DeclareMathOperator{\Prob}{Prob}
\newcommand{\Prob}[1]{\mathbb{P}[#1]}
\DeclareMathOperator{\Null}{Null}  % nullpsace
\DeclareMathOperator{\Range}{Range}     % range
\DeclareMathOperator{\Image}{Im}        % image

% functions and operators
\DeclareMathOperator{\sign}{sign}     % signum/sign of a scalar
\DeclareMathOperator{\dom}{dom}         % domain
\DeclareMathOperator{\epi}{epi}         % epigraph
\DeclareMathOperator{\argmin}{argmin}        % argmin
\DeclareMathOperator{\prox}{prox}       % proximal operator

% topology
\DeclareMathOperator{\interior}{int}    % interior
\DeclareMathOperator{\ri}{rint}         % relative interior
\DeclareMathOperator{\rint}{rint}       % relative interior
\DeclareMathOperator{\bdry}{bdry}       % boundary
\DeclareMathOperator{\cl}{cl}           % closure

% vectors, matrices
\DeclareMathOperator{\linspan}{span}
\DeclareMathOperator{\linspace}{linspace}
\DeclareMathOperator{\cone}{cone}
\DeclareMathOperator{\traceOp}{tr}           % trace
\DeclareMathOperator{\rank}{rank}       % rank
\DeclareMathOperator{\conv}{conv}       % convex hull
%\DeclareMathOperator{\Diag}{Diag}       % Diag(v) = diagonal matrix with v_i on the diagonal
    % diag(D) = the diagonal vector of matrix D
\DeclareMathOperator{\Arg}{Arg}         % Argument

% operators with parentheses
\newcommand{\diag}[1]{\mathbf{diag}\left( #1\right)}
\providecommand{\null}[1]{{\rm Null}\left( #1\right)}
\providecommand{\range}[1]{{\rm Range}\left( #1\right)}
\providecommand{\span}[1]{{\rm Span}\left\{ #1\right\}}
\providecommand{\trace}[1]{{\rm Trace}\left( #1\right)}
\newcommand{\Tr}[1]{\mathbf{Tr}\left( #1\right)}

\newcommand{\Exp}[1]{{{\rm E}}[#1] }    % expectation
%\newcommand{\inner}[1]{\langle#1\rangle}
\newcommand{\E}[1]{\mathbb{E}\left[#1\right] }
\newcommand{\Et}[1]{\mathbb{E}_t \left[#1\right] }
\newcommand{\EE}[2]{\mathbb{E}_{#1}\left[#2\right] }
\newcommand{\ED}[1]{\mathbb{E}_{\mS\sim \cD}\left[#1\right] }


\usepackage{comment}

